Globular clusters as tracers of the dark matter content of dwarfs in galaxy clusters

Globular clusters (GCs) are often used to estimate the dark matter content of galaxies, especially dwarfs, where other kinematic tracers are lacking. These estimates typically assume spherical symmetry and dynamical equilibrium, assumptions that may not hold for the sparse GC population of dwarfs in galaxy clusters. We use a catalog of GCs tagged onto the Illustris simulation to study the accuracy of GC-based mass estimates. We focus on galaxies in the stellar mass range 10$^{8} - 10^{11.8}$ M$_{\odot}$ identified in $9$ simulated Virgo-like clusters. Our results indicate that mass estimates are, on average, quite accurate in systems with GC numbers $N_{\rm GC} \geq 10$ and where the uncertainty of individual GC line-of-sight velocities is smaller than the inferred velocity dispersion, $\sigma_{\rm GC}$. In cases where $N_{\rm GC} \leq 10$, however, biases may result depending on how $\sigma_{\rm GC}$ is computed. We provide calibrations that may help alleviate these biases in methods widely used in the literature. As an application, we find a number of dwarfs with $M_{*} \sim 10^{8.5}\, M_{\odot}$ (comparable to the ultradiffuse galaxy DF2, notable for the low $\sigma_{GC}$ of its $10$ GCs) with $\sigma_{\rm GC} \sim 7$ - $15\; \rm km \rm s^{-1}$. These DF2 analogs correspond to relatively massive systems at their infall time ($M_{200} \sim 1$ - $3 \times 10^{11}$ $M_{\odot}$) which have retained only $3$-$17$ GCs and have been stripped of more than 95$\%$ of their dark matter. Our results suggest that extreme tidal mass loss in otherwise normal dwarf galaxies may be a possible formation channel for ultradiffuse objects like DF2.

==> deletedtext.tex <==

In dispersion dominated systems that are collisionless, like the population of GCs, the enclosed dark matter mass can be estimated within the Jeans formalism derived from the collisionless Boltzman equation \citep{bintre2008}. Assuming spherical symmetry, and based on the radial density distribution $n$, line-of-sight velocity dispersion $\sigma_{\rm los}$ and orbit anisotropy $\beta$ of a tracer, one can write:

\begin{equation}
    -\rm n\frac{\rm d\Phi}{d \rm r} = \frac{d(\rm n \sigma_{\rm los}^2)}{d\rm r} + \frac{2\beta \rm n \sigma_{\rm los}^2}{\rm r}
    \label{eq:jeans}
\end{equation}

\noindent where $\Phi$ is the total gravitational potential as a function of the radius r contributed by both, the luminous and the dark matter component. Unfortunately, the orbital anisotropy $\beta$ is difficult to obtain from observations of stars or GCs, adding significant uncertainties to the recovered gravitational potential and mass distribution. However, studies have shown that this uncertainty is minimal when measuring the mass at one specific point: the half mass radius of the luminous tracer \citep{Walker2009, Wolf2010}. 

Within such formalism and under assumptions of spherical symmetry and dynamical equilibrium, Eq.~\ref{eq:jeans} can be simplified to estimate the mass enclosed within the half mass radius $r_h$ following  $M(< \rm r_h) = \kappa \rm G^{-1} \sigma_{\rm los}^2 r_h$, with G the gravitational constant and $\kappa$ a constant that depends on the specific definition of $r_h$ used and underlying mass distribution assumed \citep{Walker2009,Wolf2010,Walker2011,Errani2018}. Such mass modeling has been applied successfully to estimate the mass in MW dSph and ultrafaint galaxies as well as, in more recent studies, the dark matter mass of UDGs. 
%Additionally, we can estimate dynamical mass via the scalar virial theorem, as was done in \citet{Walker2011} and \citet{Errani2018}. However, this method relies on knowing the underlying distribution of mass \textit{a priori}, which, given the evasive nature of dark matter, is usually unknown. Under certain simplifying assumptions and claiming ignorance of certain variables, the scalar virial theorem does simplify to the same simple form above where the constant k is a function of several variables related to the mass distribution. 

Besides the implicit assumptions made regarding spherical symmetry and dynamical equilibrium, both holding not entirely true within the cosmological assembly of satellite galaxies, the low number of luminous tracers when dealing with GCs is an obvious source of concern. For instance, the kinematical measurements of GCs in UDG galaxies are based on a modest number of GC spectra with confirmed association, ranging from 7 to a dozen. Idealized tests presented in \citet{Toloba2016} indicate that the uncertainties introduced by the low number of targets can be significant below $\sim 20$ GCs, and may be helped by minimizing the individual velocity errors of each tracer. While encouraging, it remains to be  seen if similar conclusions can be reached when the scarcity of tracers is combined with the evolution of galaxies within the dynamical cosmological environment of groups and clusters.



%Eq.~\ref{eq:wolf} is extremely powerful when combined with spectroscopic information of a collisionless tracer, for example stars in early type galaxies. \citet{Wolf} estimated the dark matter content of Milky Way dwarfs by measuring the velocity dispersion $\sigma_{los}$ and the light profile to determine $r_{1/2}$. Variations of this estimator have also been successfully applied to dwarfs in the Milky Way \citet{Walker2011, more??}, dwarf ellipticals in clusters and also massive ellipticals (refs??).  --- Intro

%Although traditionally Eq.~\ref{eq:wolf} is applied to stellar tracers, GCs present an attractive alternative given their relative brightness and extended radial distribution compared to the stars (see for instance Fig.~\ref{fig:rgc}). The method has been applied to estimate dynamical masses of dwarf spheroidals in the MW, dwarf elliptical galaxies, massive ellipticals and, more recently, the dynamical mass of ultra-diffuse galaxies (UDGs) (refs??).   --- Intro




with $\alpha=0.5$ and $3$ for the red and blue components, respectively 





The approach to add GCs into Illustris is reminiscent of the techniques used for studies of, for example, stellar halos in simulations that did not include a stellar component \citep{bullock2005} or the tidal evolution of dwarfs in idealized dark-matter only simulations \citep{Penarrubia2008}. In short, the method can be summarized as follows. 

GCs are added by selecting dark matter particles that follow a Hernquist profile \citep{hernquist1990}:

\begin{equation}
    \rho_{\rm HQ} = \frac{\rho_{\rm HQ}^0}{(\rm r/\rm r_{\rm HQ})(1 + \rm r/\rm r_{\rm HQ})^3}
    \label{eq:hq}
\end{equation}

\noindent 
where $\rho_{\rm HQ}^0$ is the characteristic density and r$_{\rm HQ}$ is the scale radius.  % $\beta r_{\rm NFW}$where $\beta$ depends on the population of GCs being tagged.
The original tagging includes a blue, metal poor and extended GC component plus a population of red, metal rich more spatially clustered GCs with fractions that reproduce observations \citep{Harris2017}. However, in this paper we do not make any distinction between these two components.

The dark matter halo of infalling galaxies is approximated by the best-fit NFW profile \citep{Navarro1996}:

\begin{equation}
    \rho_{\rm NFW} = \frac{\rho_{\rm NFW}^0}{(\rm r/\rm r_{\rm NFW})(1 + \rm r/\rm r_{\rm NFW})^2}
    \label{eq:nfw}
\end{equation}

\noindent 
where $\rho_{\rm NFW}^0$ is the characteristic density and r$_{\rm NFW}$ = r$_{\rm max}/2.1623$ is the scale radius, and r$_{\rm max}$ is the radius of maximum circular velocity. 

To determine the set of candidate dark matter particles that follow the desired GC distribution, we compare the actual distribution function of the dark matter $f_{\rm DM}$, calculated from the particle data, to the target distribution function of GCs $f_{\rm GC}(\epsilon)$, calculated from the tracer of profile $\rho_{HQ}$ embedded in a gravitational potential of the NFW dark matter component. In other words, the distribution function of GCs follows: 

\begin{equation}
    f_{\rm GC}(\epsilon) = \frac{1}{8\pi}\bigg[ \int_{0}^{\epsilon} \frac{\rm d^2\rho}{\rm d\psi^2} \frac{\rm d \psi}{\sqrt{\epsilon - \psi}} + \frac{1}{\sqrt{\epsilon}} \bigg(\frac{\rm d\rho}{\rm d\psi}\bigg)_{\psi = 0}\bigg]
    \label{eqn:distfunc}
\end{equation}

\noindent 
where $\rho = \rho_{\rm HQ}$ and represents the density of the GCs, $\Psi$ is the gravitational potential of the NFW halo (GCs and baryons are assumed sub-dominant) and $\epsilon$ is the relative energy of the particles in the halo. Globular cluster candidate particles are then selected by randomly choosing a fraction f$_{\rm GC}$/f$_{\rm DM}$ of the particles within bins of relative energy. 

This exercise identifies all dark matter particles that follow the target distribution of GCs. The scale lengths of the Hernquist profile are chosen such that $r_{\rm HQ} = \alpha r_{\rm NFW}$, with $\alpha=0.5$ and $3$ for the red and blue components, respectively. Additionally, to avoid GCs systems that are too extended, only dark matter particles within $3r_h$ are consider eligible, where $r_h$ is the half-mass radius of the dark matter halo. These choices were made to reproduce observations of GCs around $L_*$ galaxies, see \citet{ramalm2020} for details. 

This procedure is designed to maximize the number of tracers that are possible GC candidates. As a result, each galaxy contains a variable number of particles that are GC candidates and, in the large majority of cases, exceeds the realistic number of GCs expected. The last ingredient of the method is to calibrate the equivalent GC-mass for each of these tagged particles such that the galaxies are, at $z=0$, consistent with the observed relation between halo mass and GC mass \citep{Harris2015}. This relation has the form $M_{GC} = a M_{200}^b$ with $a=4\times 10^{-5}$ and $b=1.03$. %\textcolor{cyan}{Should we cite the red/blue parameters individually or the relation using all GCs?} \lvs{the one for all}

Note that, after infall, galaxies may experience tidal removal of mass (and also GCs) by the gravitational potential of the cluster, a process naturally accounted for by our numerical simulations. The mass calibration takes this process into account by calibrating the \citet{Harris2015} relation upwards (at infall) to account for this stripping \citep[see ][ for details]{ramalm2020}.
\lvs{Details on the calibration: to calibrate the infall parameters ($a_{\rm inf}, b_{\rm inf}$) we performed a least-square-fit to the observational relation $M_{\rm GC} = a * M_{vir,0}^b$, with ($a,b$) given by Harris et al. 2015. More specifically, we compute for each galaxy the fraction of candidate GCs ($f$) that remain bound to the object at $z=0$. Then, using the infall virial mass and the one estimated at z=0 (from abundance matching, Hudson 2015), we find ($a_{\rm inf}, b_{\rm inf}$) by a least-square-fit to the following relation: 
$M_{\rm GC,inf} = a_{\rm inf} * M_{\rm vir,inf}^{b_{\rm inf}} = (1/f) * a_0 * M_{\rm vir,0}^{b_0}$,  where $a_0$ and $b_0$ corresponds to the $z=0$ observed values by \citet{Harris2015}.}


Since typically the number of candidate GCs particles is larger than observed number of GCs per galaxy, the mass assigned to each tagged GC is typically much smaller than an actual GC. When needed, we will refer to a "realistic" number of GC per galaxy, which is computed by dividing the total GC mass in that galaxy by a fixed average mass assumed per GC $m_{\rm GC} = 10^5$\msun.


